On the Centre of Strong Graded Monads

We introduce the notion of 'centre' for pomonoid-graded strong monads which generalizes some previous work that describes the centre of (not graded) strong monads. We show that, whenever the centre exists, this determines a pomonoid-graded commutative submonad of the original one. We also discuss how this relates to duoidally-graded strong monads.

==> related.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{sec:related}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This work takes direct intuitions from \cite{central-submonads} and \cite{canonical}.
In fact, for the construction on monadic part of the centre of graded monads,
it is necessary to use similar constructions as in \cite{central-submonads},
including the similar theorems, definition of graded central cone,
and proof strategy of the centre Theorem.
Another related work concerning the monadic part is \cite{premonoidal},
they give the \emph{central morphism} and \emph{premonoidal centre}. 
Nonetheless, our approach in this part 
has no connection with that as we deliberately avoid the utilization of Kleisli constructions.

To construct the centre, we have to first study commutativity. 
\cite{GARNER} describes a general framework for commutativity based on enriched category theory, 
and preprint \cite{commu-graded-22} gives definition of commutative graded monads,
and it is as far as we know the only work yet discussing commutativity of graded monads.
However, its definition relies on their previous work of \emph{suspension} of a monoidal category.

For the gradation part, \cite{canonical} defined graded monads as lax monoidal functors
between skew monoidal categories, which is more general than those between monoidal categories 
due to less monoidal property requires, and defined the morphisms between them. 
It exceeds the scope of our work since our focus so far being monoid graded monads on monoidal category, 
but it is where we draw inspiration for the definition of the morphisms between strong graded monads.
While other definitions exist for morphisms between graded monads, 
many of them lack the required generality to be applicable to our context.
For example \cite{Unifying20} gives morphisms and transfers between graded monads that are graded by same category.
But they do not give the definition of strong graded monads, nor the morphisms between different gradations. 
Our construction of morphism between strong graded monads in Definition \ref{def:morph-monad-graded} is 
novel.

